Long-HOT: A Modular Hierarchical Approach for Long-Horizon Object Transport

We address key challenges in long-horizon embodied exploration and navigation by proposing a new object transport task and a novel modular framework for temporally extended navigation. Our first contribution is the design of a novel Long-HOT environment focused on deep exploration and long-horizon planning where the agent is required to efficiently find and pick up target objects to be carried and dropped at a goal location, with load constraints and optional access to a container if it finds one. Further, we propose a modular hierarchical transport policy (HTP) that builds a topological graph of the scene to perform exploration with the help of weighted frontiers. Our hierarchical approach uses a combination of motion planning algorithms to reach point goals within explored locations and object navigation policies for moving towards semantic targets at unknown locations. Experiments on both our proposed Habitat transport task and on MultiOn benchmarks show that our method significantly outperforms baselines and prior works. Further, we validate the effectiveness of our modular approach for long-horizon transport by demonstrating meaningful generalization to much harder transport scenes with training only on simpler versions of the task.

==> figures/data_statistics_old.tex <==
\begin{figure*}[t]
    \centering
    \rotatebox[origin=c]{90}{\makebox[1in]{Standard Long-HOT}}%
    \begin{subfigure}{0.30\textwidth}
        \includegraphics[]{pics/data_statistics/small_scale_transport_3_train.png}
        \caption{Train}
        \label{subfig:train-stat}
    \end{subfigure}
    \begin{subfigure}{0.30\textwidth}
        \includegraphics[]{pics/data_statistics/small_scale_transport_3_test.png}
        \caption{Val}
    \end{subfigure}
    \begin{subfigure}{0.30\textwidth}
        \includegraphics[]{pics/data_statistics/small_scale_transport_3_val.png}
        \caption{Test}
    \end{subfigure}
    
    \rotatebox[origin=c]{90}{\makebox[1in]{Large Long-HOT}}%
    \begin{subfigure}{0.30\textwidth}
        \includegraphics[]{pics/data_statistics/hard_transport_10_val.png}
        \caption{\textit{default} - test data}
    \end{subfigure}
    \begin{subfigure}{0.30\textwidth}
        \includegraphics[]{pics/data_statistics/hard_transport_8_val.png}
        \caption{\textit{hard} - test data}
    \end{subfigure}
    \begin{subfigure}{0.30\textwidth}
        \includegraphics[]{pics/data_statistics/hard_transport_9_val.png}
        \caption{\textit{harder} - test data}
    \end{subfigure}
    \caption{Shows the statistics of the episodes used in Long-HOT. The x-axis represents geodesic distance of a reference trajectory in meters and y-axis shows fraction of total episodes in the corresponding histogram bin. 
    (a) represents statistics of the episodes used to train all methods. (c, d, e and f) show test data statistics used in standard and large Long-HOT settings. Geodesic distance of the reference trajectories in Large Long-HOT, indicates increasing task complexity of test scenarios where agent's require deeper exploration and long-horizon planning to complete the task.
    % As seen the task configurations used in Large Long-HOT show the increasing task complexity in terms of required exploration and  
    }
    \label{fig:dataset_statistics}
    
\end{figure*}

% \begin{table*}[]
% \begin{tabular}{c|l|l|l|}
% \rotatebox{90}{Standard Long-HOT}
% & \includegraphics[width=0.30\textwidth]{pics/data_statistics/small_scale_transport_3_train.png}
% & \includegraphics[width=0.30\textwidth]{pics/data_statistics/small_scale_transport_3_test.png}
% & \includegraphics[width=0.30\textwidth]{pics/data_statistics/small_scale_transport_3_val.png}\\
% \midrule
% \rotatebox{90}{Large Long-HOT}
% & \includegraphics[width=0.30\textwidth]{pics/data_statistics/hard_transport_10_val.png}
% & \includegraphics[width=0.30\textwidth]{pics/data_statistics/hard_transport_8_val.png}
% & \includegraphics[width=0.30\textwidth]{pics/data_statistics/hard_transport_9_val.png}\\
% \end{tabular}
% \end{table*}


==> rebuttals/comments.tex <==
Reviewers find our paper to be ``well written'' (\ra, \rc), deem both Long-HOT and HTP to be ``challenging'' (\rd) and ``interesting'' (\rb) for long-term autonomy where our method performs ``very well'' (\ra).
We appreciate the feedback and will incorporate all comments in the final version.
%We appreciate the thoughtful feedback, and address their questions below.



\vspace{0.1cm}
\noindent {\bf Code release} [\ra, \rc]. As mentioned in the supplementary, all the code and data for this paper will be released.


\vspace{0.1cm}
\noindent {\bf Mapping and localization of HTP} [\ra, \rb]. 
We do not assume access to map nor allow agent to gather information prior to the task. But similar to previous works like [6,13,28,36] we allow access to pose for agent localization. Moreover for simplicity and faster training speeds, instead of creating a depth projected occupancy every timestep, we use a pre-built occupancy map that is only revealed to a maximum of 5m (no object information) and use ray tracing to avoid revealing more when occlusions are involved.

% We do not assume access to map nor allow agent to gather information prior to the task. But similar to previous works like [6,13,28,36] we allow access to pose for agent localization. Moreover for simplicity and faster training speeds, instead of creating a depth projected occupancy every timestep, we use a pre-built occupancy map that is only revealed to a maximum of 5m (no object information) and use ray tracing to avoid revealing more when occlusions are involved.

\vspace{0.1cm}
\noindent \textbf{Distinction of Long-HOT from Puig et al.~[A1,A2]} [\rb]. 
Our contributions are orthogonal to works like VirtualHome [A1] or Watch and Help [A2]. VirtualHome is an embodied AI task that focuses on breaking down complex language instructions or videos into programs that can be executed by an embodied agent. {\em VirtualHome abstracts both navigation and interaction} and the embodied agent is only a means to verify the generated program. Methods developed to solve Long-HOT are complementary to [A1,A2] as they help in realising long-horizon navigation of agents. 
\blfootnote{A1. Puig. et al, “VirtualHome: Simulating household...”, CVPR 2018}
\blfootnote{A2. Puig. et al, “Watch-and-help: A Challenge for...”, ICLR 2021}

\vspace{0.1cm}
\noindent \textbf{Distinction from navigation benchmarks} [\rb, \rd]. 
Long-HOT is ``more complex'' (\rc) and ``goes beyond existing navigation benchmarks'' (\ra) where commonly used flat policy architectures [36] fail completely as seen in Table 3.
% As shown in Table 3, while embodied navigation methods commonly use flat policy architectures [36], they fail completely on Long-HOT. 
This shows Long-HOT's potential to serve as a testbed for novel architectures for planning, exploration and reasoning over long spatial and temporal horizons. 

% \vspace{0.1cm}
% \noindent \textbf{Distinction from navigation benchmarks} [\rb, \rd]. 
% As shown in Table 3, while embodied navigation methods commonly use flat policy architectures [36], they fail completely on Long-HOT. This shows Long-HOT's potential to serve as a testbed for novel architectures for planning, exploration and reasoning over long spatial and temporal horizons. 

%\noindent \textbf{Importance of Long-HOT benchmark.} [\rb,\rd] First, we would like to point out that our contributions are orthogonal to works like VirtualHome[A1] or Watch and Help[A2] mentioned by [\rb]. VirtualHome is an embodied AI task which focuses on breaking down complex language instructions or video sequences into programs that can be executed by an embodied agent. There, both the navigation and interaction parts are abstracted and the embodied agent is only used as a means to verify the generated program. In fact, methods developed to solve LongHOT are complementary to the prior benchmarks[A1,A2] as they help in realising long-horizon navigation of agents. Further as shown in Table 3, while embodied navigation methods commonly use flat policy architectures [36], such architectures fail completely on Long-HOT. This shows Long-HOT's potential to serve as a testbed for, and accelerate the development of novel architectures for planning, exploration, and reasoning over long spatial and temporal horizons. \blfootnote{A1. Puig. et al, “VirtualHome: Simulating household...”, CVPR 2018}
% \blfootnote{A2. Puig. et al, “Watch-and-help: A Challenge for...”, ICLR 2021}


\vspace{0.1cm}
\noindent \textbf{Task specific method.} [\rb] 
HTP is a generic hierarchical structure for long-horizon navigation. Its components like topological graph, object-nav and exploration can be easily transferred to other tasks. While the high-level controller is heuristic, it would be interesting to see how a learned controller optimizes between efficiency and task execution. 
%Further, such hierarchies also provide an easy way to bridge outputs from works like [A1,A2] to perform long-horizon execution.


% From Table 3 (left) we can see that combining learning with planning like HTP (which uses MP for point goals within explored regions and RL policies for semantic targets at unknown locations) is robust towards imperfect hand-offs and fares better in comparison to alternative hierarchical approaches like [21,40] that only set waypoints for navigation.

% \vspace{0.1cm}
% \noindent \textbf{Insights on modularity} [\rb]. 
% While hierarchical models have addressed these topics before, not all hierarchical methods provide sufficient gains. From Table 3 (left) we can see that combining learning with planning like HTP (which uses MP for point goals within explored regions and RL policies for semantic targets at unknown locations) is robust towards imperfect hand-offs and fares better in comparison to alternative hierarchical approaches like [21,40] that only set waypoints for navigation.
% (more details at L588-600).

% \vspace{0.1cm}
% \noindent \textbf{Insights from HTP.} [\rb] 
% While the insights in terms of modularity and generalization of hierarchical models have been studied before, not all hierarchical architectures provide sufficient gains. From Table 3 (left) we can see that combining learning with planning like HTP (which uses MP for point goals within explored regions and RL policies for semantic targets at unknown locations) is robust towards imperfect hand-offs and fares better in comparison to alternative hierarchical approaches like [21,40] that only set waypoints for navigation (more details at L588-600).


% \vspace{0.1cm}
\noindent \textbf{Analysis on container usage.} [\rb] 
% \nn{Waiting for training to be done. The values I've put are from an intermediate checkpoint. Will update the exact values by Sunday morning. But I believe the trends might not change too much.}
We analyse the container usage and policies in Tab.~\ref{tab:container_table} and Fig.~\ref{fig:container_pickup}. We see that adding an incentive for picking up a container improves SPL \& PPL metrics for both methods, indicating efficiency in task execution. Further, NoMap's container usage is higher than OracleMap methods indicating that NoMap policies prefer picking up a container due to the uncertainties involved in the location of target objects, while OracleMap methods are aware of target object locations and container usage becomes more selective. 
Having zero objects at the goal while the container was picked up shows that agent executes behaviors like dropping already picked up objects for efficiency. 
% \jd{This point is hard to understand (and also Fig R1 is quite hard to parse.)}
% we can infer that agents also execute behaviors like dropping target objects to pickup a container for efficiency.
% Table \ref{tab:container_table} shows the container usage and performance of baseline methods. Fig. \ref{fig:container_pickup} shows when the agent decided to pickup the container.....
We will add this in final version.
% This includes cases where the agent picked up an object and decided 

\input{rebuttals/container_results}
\input{rebuttals/container_pickup}


\vspace{0.1cm}
\noindent \textbf{Insights on modularity} [\rb]. 
While hierarchical models have addressed these topics before, ``not all'' (\rc) hierarchical methods provide sufficient gains. 
% We answer questions like ``Are hierarchies good? (yes, but not all)'' (\rc). 
From Table 3 (left) we can see that combining learning with planning like HTP (using a combination of MP and RL policies) is robust towards imperfect hand-offs and fares better in comparison to alternative hierarchical approaches like [21,40] that only set waypoints for navigation.


\vspace{0.05cm}
\noindent \textbf{HTP's performance on benchmarks.} [\rd] 
% HTP provides significantly better performance than baselines on Long-HOT and on par performance with [24] on MultiON[36]. 
HTP provides significantly better performance on Long-HOT and on par performance with [24] on MultiON [36]. HTP uses weighted frontier exploration technique that comes with theoretical exploration guarantees hence, its significance is a lot higher in a long-horizon transport like Long-HOT compared to MultiOn where end-to-end RL methods fail. 


\vspace{0.05cm}
\noindent \textbf{Clarification on HTP's exploration.} [\rb] 
The policy uses closeness scores to reach a node close to the previously observed object. The threshold in closeness scores is dropped when there are no more frontiers and the agent iterates through nodes with highest scores for the target.

\vspace{0.05cm}
\noindent \textbf{Details on rewards.} [\rb, \rd] 
% The rewards for the policies have been carefully assigned after several iterations. 
The weighting between the rewards can be assumed to be implicit in the reward value. We will put the values in supp. and also release the code.

\vspace{0.05cm}
\noindent \textbf{Large indoor environments.} [\rc] We specify a scene to be large if at least one of its dimensions is greater than $40m$. In Table 3 (left) we only consider such large environments. 

%\vspace{0.05cm}
%\noindent \textbf{Typos, corrections and suggestions} [\ra,\rb,\rc]. Thank you, we will incorporate all comments in the final version.

\vspace{0.05cm}
\noindent \textbf{LongHOT+} [\rc]. 
Indeed, we will add discussion for multi-agent scenarios, work-energy constraints for transport, etc.

\vspace{0.05cm}
\noindent \textbf{Complementary [24]} [\rc]. We will add discussion for how  auxiliary tasks may improve HTP akin to object navigation.

% \noindent\textbf{Reviewer 1}
% \review{
% \begin{itemize} \itemsep -2pt
%     \item My main issue regarding this submission is about an aspect of the proposed method that I don’t understand - I’m especially concerned about whether this aspect leads to an unfair comparison to other methods in this space. Maybe I missed it but I am a bit confused about how localization and mapping is happening in the proposed approach. My understanding is that the agent only has access to RGBD input, not its position in the map or the map itself. But both seem to be necessary for the approach - how are these generated? Does this assume that the agent can gather information about a scene before the actual task? Do all other methods that are used as baselines for the new and the existing benchmark have access to the same information?
    
%     \item Since the new benchmark is one of the main contributions, it is important that others can test their methods in it. I did not find a statement in the paper about sharing the code. Can the authors please confirm that the benchmark will be made available upon submission?
% \end{itemize}
% }


% \vspace{0.2cm}
% \noindent\textbf{Reviewer 3}

% \review{
% \begin{itemize}\itemsep -2pt
%     \item \textbf{Benchmark:} While the authors claim that they include object transport compared to previous navigation benchmarks, they fail to mention a previous benchmark environment on embodied AI that offers the possibility to study exactly such tasks [1]. The only real difference I see is that in this submission, the agent can carry multiple objects and find a container that allows to carry even more objects. However, this aspect is not really properly evaluated in this paper.
%     \item Similarly to this submission, VirtualHome also abstracts away physical reasoning of atomic actions to focus on more complex, long-horizon tasks.
%     \item Hence, much of the claimed novelty on the benchmark is diluted unless the authors can provide a convincing discussion why their environment is fundamentally different.
%     \item For these reasons, I feel like the authors should tone down their claims about the benchmark’s novelty and focus on their method.
%     \item Examples of agents that navigate partially observable environments and pick-up objects and move them to other locations are proposed in [2]. A difference I can see in the settings is that in this submission, the topological map is created during exploration, while it is already predefined for the agents in [2]. This trade-off between exploration and task solving should really become the focus of this paper in my opinion.
%     \item \textbf{Method:} Overall, I find the proposed approach too task-specific. While a modularized approach to functionally separate tasks makes sense, it contains a lot of hand-crafted modules with specialized components and cost functions that are combined together to make the whole system work for this specific task. For instance, a high-level heuristic based module controls which of the submodules is used (explore, pickup, drop). It would be much better to frame this in a more general manner, i.e., instead of the pickup and drop, why not formalize it as a more general action set that can be executed besides exploration (e.g., multiple interactions with objects and the environment). Moreover, in its current state, the heuristics need to be defined for each new task. If one could learn this via interactions with the environment directly, the issue could be alleviated.
%     \item The insight that modular separation leads to improved performance is not new and has been studied for a long time, e.g., in the context of hierarchical reinforcement learning [3]. Especially in robotics, such modular approaches have recently been shown to generalize to harder settings during inference which is claimed as one of the insights of this work, e.g., in the context of waypoint finding for autonomous driving [4], navigation tasks with 2D maps [5] or for long-horizon robotic manipulation tasks [6].
%     \item I would recommend the authors to focus on one solution for the exploration score prediction, which would help the flow of the paper (the alternative option could be mentioned in the supplementary material).
%     \item One thing that is unclear to me from the paper is what happens if the agent has dropped off objects and needs to collect more (assuming it did not find the container), does it go back to exploring unseen frontiers (even if the objects had been detected already but not picked up due to load constraints) or is there a way to directly go to the object, even if the object closeness score is below a certain threshold? Also, how does the exploration work if the environment has been fully explored, i.e., if there are no more frontiers? Maybe this is related to the (undefined) “node subgoal” in Fig. 3.
%     \item While there are important questions raised, such as “having found an object far from the goal, should an agent immediately return to drop it off at the goal, or should it look for another object before returning for efficiency?” (L206-208), they are not properly answered and discussed in the experiments. It would be important to include evaluations to analyze the agents’ behavior. Also, it would be interesting to see whether the policy actually learns to pick up the container to be more efficient, i.e., whether it performs a greedy transport if it sees the goal or explores more to find the container (as stated on L134-136).
%     \item Are there no weights used for equation 1 and 2 to balance the different reward terms? If not, I would imagine the time penalty to quickly outweigh the other rewards.
%     \item L350: how is a collision with the environment defined?
%     \item L359: Can you clarify how the pre-built occupancy map is defined?
%     \item L530: should it not be Gref/Gpl, because if the actual path length (Gpl) is longer than the reference path (Gref), the SPL should decrease.
%     \item Table 3: the baseline’s scores are on par with the author’s score, but only the latter are marked as bold. Also the claim on L613-614 “is nearly on par or better” is false, it is “on par or worse” than the baseline. This needs to be corrected.
%     \item Fig 4: it is hard to understand what’s shown in this figure. What happens between the 2nd and 3rd instance (from left to right)? Have the picked up objects (blue, red) already been moved to goal? It seems like there are some in-between steps missing.
%     % \item Fig. 4 caption (and in the text): I think it would be easier if the authors use the term “goal location” instead of “goal object” as the drop-off location.
%     % \item The bibliography needs to be cleaned up, it is very inconsistent and incomplete. For example, some references miss the publication venue and have the wrong dates, e.g., [16] is from 2017 and was published in CVPR or [3] should be 2016 and was published in AAAI. There are more examples, which I won’t list here.
%     % \item The provided video contains a lot of lag and is quite overloaded. There is definitely a lot of room for improvement.
% \end{itemize}
% }

% While the high-level controller is heuristic it provides an easy way to connect the outputs from works like [VirtualHome or Watch-and-Help] for long-horizon task execution. 
% \nn{needs to be more specific.}
% Our aim through HTP is to actually present an hierarchical structure that is general in tackling different long-horizon problems rather than learning a task specific policy for every high level behavior. The majority of the components in HTP like topological graph, object navigation and exploration can be readily transferred to other tasks. While the High-level controller in our work is heuristic, 

% Please refer to L588-600 for more details. 

% While the insights in terms of modularity and generalization of hierarchical models have been studied before and hierarchical models generally fare better, it is worth noting that not all hierarchical architectures provide sufficient gains. For instance, with hierarchies such as [21,40] where the expressivity of subgoals is largely limited to goal reaching for navigation performs worse in comparison to HTP (Table 3 Left).
% and hierarchical models fare better than flat policy architectures in such scenarios


% In case of an already observed object that was not picked up due to the load constraints, the agent directly travels to the node closest to the object and activates the object-nav policy. The threshold in closeness scores for object is dropped when there are no more frontiers to explore and the agent by default stays in pick-drop stage where it iterates through the nodes with highest scores for the target object. 
% Further, our object navigation policy is also robust to imperfect handoffs as seen in HTP w/o graph from Fig 1 (in supp.).

% If the agent has already observed an object but did not pickup due to the load constraint, it directly goes to the node-location where the object was observed and activates the object-nav policy. The closeness score threshold is only present to eliminate any false positives but is dropped when there are no frontiers to explore. The agent by default goes into Pick-Drop situation where it iterates through the nodes with highest scores for the object and calls the object navigation policy. 


% \vspace{0.2cm}
% \noindent\textbf{Reviewer 4}

% \review{
% \begin{itemize} \itemsep -2pt
%     \item In my opinion, there are no strong weak points, with respect to what the paper claims to be focusing on. On the other hand, I would suggest clarifying a bit some of the points mentioned in the paper. For instance:
%     \item For general readers, it is convenient to state what is a large indoor environment and what is not. Are we talking just about square meters, or also about having more or fewer rooms, or … ? Some sentences about this would be worth being included in the introduction. And give some quantitative comparison of Long-HOT wrt MultiON in this regard, which could be done either in the “related work” section or the “experiments” one.
%     \item From the paper, it seems that all collected objects must be dropped at the same location. Perhaps, dropping different objects in different locations maybe even a more challenging task if time-to-completion is considered. Would this make sense as a new task? (a sort of Long-HOT+). If so, it could be mentioned as future work.
%     \item It is stated that [24] is complementary to the agent proposed in this paper. It would be good to add some hints about this in a couple of sentences.
% \end{itemize}
% }


% \vspace{0.2cm}
% \noindent\textbf{Reviewer 5}

% \review{
% \begin{itemize} \itemsep -2pt
%     \item Even though the new task is challenging, it still falls into the type of navigation + task which has been explored by many previous work. Simply adding a container seems not convincing enough to claim that it is a contribution of new task.
%     \item Some implementation details are missing. For the policy part, i.e. eq. 2, simply adding up the rewards of different sources and units seems not convincing. Also, if you use the alogrithm of PPO, why still needs a rslack for time penalty?
%     \item The performance is not promsing enough. The core contribution from my understanding is a new GCN-based hierarchical model. However, Tab. 2 (left) does not show that HTP-GCN has any advantages. In Tab. 2 (right), the algorithm proposed by the work is in fact inferior to [24]. I do not think the proposed method can address the challenges as they claim in line 010.
% \end{itemize}
% }

% \vspace{0.1cm}
% \noindent \st{\textbf{Importance of LongHOT.}} [\rb, \rd]

% \vspace{0.1cm}
% \noindent \st{\textbf{Implementation details for the policy.}} [\rd]


==> rebuttals/container_pickup.tex <==
\begin{figure}[t]
    \centering
    \vspace{-0.4cm}
    \includegraphics[width=1.0\linewidth, trim={0 4.2cm 6cm 0}, clip]{pics/container_histogram.png}
    \vspace{-0.75cm}
    \caption{\small Breakdown of container usage from Tab.~\ref{tab:container_table} based on number of objects picked before container. In every column more shaded regions represent larger number of objects already at goal.
    }
    \vspace{-0.6cm}
    \label{fig:container_pickup}
\end{figure}

==> rebuttals/container_results.tex <==
\begin{table}[!!t]
\resizebox{\linewidth}{!}{
\tiny
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Model                       & \%S & \%P & SPL & PPL & \%C \\ \hline
% NoMap(w/o c-reward)                       & 17 & 42 & 11 & 19 & 57 \\
NoMap(w/o c-reward)                       & 26 & 47 & 15 & 21 & 55 \\
% NoMap(w c-reward)                       & 17 & 43 & 12 & 21 & 65 \\
NoMap(w c-reward)                       & 28 & 48 & 16 & 23 & 70 \\
% NoMap(w c-reward)                   & 37 & 55 & 22 & 27 & 70 \\
OracleMap(w/o c-reward)                       & 77 & 84 & 62 & 64 & 48 \\
OracleMap(w c-reward)                       & 81 & 88 & 67 & 70 & 50 \\
% OracleMap(w c-reward)                       & 65 & 76 & 52 & 56 & 41 \\
% OracleMap(w c-reward)                   & 88 & 92 & 72 & 73 & 43\\
\hline
\end{tabular}
}
\vspace{-0.4cm}
\caption{\small Analysis on container usage and performance on 500 test episodes with and without the incentive for picking up the container. Here, S-success, P-progress and C-container pickup \%.}
\label{tab:container_table}
\end{table}

==> tables/hard_transport_results.tex <==
\begin{table*}[]
\resizebox{\linewidth}{!}{
\tiny
\begin{tabular}{clcccccc}
\toprule
&Model                                     & \%Success$\uparrow$ & \%Progress$\uparrow$  & SPL$\uparrow$ & PPL$\uparrow$  & Episode energy$\downarrow$ & \%Picked$\uparrow$ \\ \midrule
\parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{Default}}}
& OracleMap (Occ) & 26     & 45         & 18 & 27 & 0.58    & 49\\
& OracleMap (Occ+Obj) &  85      & 91         & 65 & 67 & 0.10      & 92       \\
& OracleMap-Waypoints & 80 & 88 & 38 & 39 & 0.17 & 92\\
& NoMap & 39      & 59         & 25 & 31 & 0.45      & 62       \\
& HTP-NearestFrontier & 41 & 54 & 17 & 20 & 0.65 & 66\\
& HTP-GCN & 46 & 58 & 19 & 22 & 0.57 & 68\\
% & HTP-GCN\\
& HTP-CNN                       & {\bf 55}    & {\bf 68}    & {\bf 26}    & {\bf 30} & {\bf 0.46} & {\bf 79}\\
\midrule
\parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{Hard}}}
& OracleMap (Occ) & 3.6   & 17    & 2.3   & 10 & 0.84 & 19\\
& OracleMap (Occ+Obj) & 46      & 69         & 29 & 38 & 0.36      & 71       \\
& OracleMap-Waypoints & 48 & 72 & 18 & 24 & 0.33 & 81\\
& NoMap & 5.2      & 24         & 2.6 & 10 & 0.79      & 28       \\
& HTP-NearestFrontier & 22 & 40 & 8.1 & 14 & 0.69 & 57\\
& HTP-GCN & 27 & 47 & 9.4 & 16 & 0.59 & 60\\
& HTP-CNN                              & {\bf 33}      & {\bf 53}         & {\bf 13} & {\bf 20}   & {\bf 0.52}      & {\bf 66}        \\
\midrule
\parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{Harder}}}
& OracleMap (Occ) & 2     & 12    & 1.3   & 7.7   & 0.89  & 14\\
& OracleMap (Occ+Obj) & 26      & 48         & 16 & 26 & 0.57      & 51       \\
& OracleMap-Waypoints & 31 & 59 & 12 & 19 & 0.46 & 71\\
& NoMap & 2.8      & 16         & 1.3 & 8.0 & 0.86      & 21       \\
& HTP-NearestFrontier & 15 & 32 & 5.5 & 12 & 0.74 & 52\\
& HTP-GCN & {\bf 22} & 39 & 8.0 & 14 & 0.65 & 54\\
& HTP-CNN                              & 21      & {\bf 42}         & {\bf 8.6} & {\bf 16}   & {\bf 0.63}      & {\bf 57}        \\ \bottomrule
\end{tabular}
}
\caption{\textbf{Long Transport Task:} Shows generalizability of methods to more difficult settings within the same task. 
The methods were tested on 26 habitat scenes with at least one dimension $>40m$. All methods were trained on dataset generated with \textit{default} specification (max. radius 15m) and tested on \textit{hard} (max. radius 20m) and \textit{harder} (max. radius 30m) transport settings.}
\label{tab:deep_transport}
\end{table*}


==> tables/htp_ablation.tex <==
\begin{table}[]
\caption{Ablation }
\label{tab:multion}
\centering
% \resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
Model & \%Success$\uparrow$ & \%Progress$\uparrow$  & SPL$\uparrow$ & PPL$\uparrow$\\\midrule
OracleMap (Occ) & 16 & 36 & 12 & 27\\
OracleMap (Occ+Obj) & 48 & 62 & 38 & 49\\
NoMap               & 10 & 24 & 4 & 14 \\
FRMQN\cite{frmqn} & 13 & 29 & 24 & 24\\
SMT\cite{fang2019scene} & 9 & 22 & 7 & 18\\
ProjNeuralMap\cite{wani2020multion} & 27 & 46 & 18 & 31\\
ObjRecogMap\cite{wani2020multion} & 22 & 40 & 17 & 30\\
Lyon\cite{marza2021teaching} & 57 & 70 & \textbf{36} & \textbf{45}\\
HTP-CNN (Ours) & 56 & 69 & 30 & 36\\
HTP-GCN (Ours)& \textbf{57} & \textbf{70} & 27 & 33 \\
\bottomrule

\end{tabular}
% }
\end{table}

==> tables/largeLHOT_horizontal.tex <==
\begin{table}[]
\caption{\textbf{Large Long-HOT Task:} Shows generalizability of methods to more difficult settings within the same task. 
The methods were tested on 26 habitat scenes with at least one dimension $>40m$. All methods were trained on dataset generated with \textit{default} task configuration (max. radius 15m) and tested on \textit{hard} (max. radius 20m) and \textit{harder} (max. radius 30m) transport settings.}
\label{tab:deep_transport}
\centering
% \resizebox{\linewidth}{!}{
\begin{tabular}{c ||c|c|c|c|| c|c|c|c|| c|c|c|c}
\toprule
Model & \multicolumn{4}{c||}{Default} & \multicolumn{4}{c||}{Hard} & \multicolumn{4}{c}{Harder}\\ \midrule
\multicolumn{13}{c}{$\|$ \%Success$\uparrow$ $\vert$ \%Progress$\uparrow$  $\vert$ SPL$\uparrow$ $\vert$ PPL$\uparrow$ $\|$ }\\ \midrule
OracleMap (Occ) & 26     & 45         & 18 & 27 & 3.6   & 17    & 2.3   & 10 & 2     & 12    & 1.3   & 7.7\\
OracleMap (Occ+Obj) &  85      & 91         & 65 & 67 & 46      & 69         & 29 & 38 & 26      & 48         & 16 & 26\\
OracleMap-Waypoints & 80 & 88 & 38 & 39 & 48 & 72 & 18 & 24 & 31 & 59 & 12 & 19\\
NoMap & 39      & 59         & 25 & 31 & 5.2      & 24         & 2.6 & 10 & 2.8      & 16         & 1.3 & 8.0\\
HTP-NearestFrontier & 41 & 54 & 17 & 20 & 22 & 40 & 8.1 & 14 & 15 & 32 & 5.5 & 12\\
HTP-CNN                       & {\bf 55}    & {\bf 68}    & {\bf 26}    & {\bf 30} & {\bf 33}      & {\bf 53}         & {\bf 13} & {\bf 20} & 21      & {\bf 42}         & {\bf 8.6} & {\bf 16}\\
HTP-GCN & 46 & 58 & 19 & 22 & 27 & 47 & 9.4 & 16 & {\bf 22} & 39 & 8.0 & 14\\
\bottomrule
\end{tabular}
% }
\end{table}


==> tables/long_transport_minimal.tex <==
\begin{table}[]
\caption{\textbf{Large Long-HOT Task:} Shows generalizability of methods to more difficult settings within the same task. 
The methods were tested on 26 habitat scenes with at least one dimension $>40m$. All methods were trained on dataset generated with \textit{default} task configuration (max. radius 15m) and tested on \textit{hard} (max. radius 20m) and \textit{harder} (max. radius 30m) transport settings.}
\label{tab:deep_transport}
\centering
% \resizebox{\linewidth}{!}{
\begin{tabular}{clcccc}
\toprule
&Model                                     & \%Success$\uparrow$ & \%Progress$\uparrow$  & SPL$\uparrow$ & PPL$\uparrow$\\ \midrule
\parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{Default}}}
& OracleMap (Occ) & 26     & 45         & 18 & 27\\
& OracleMap (Occ+Obj) &  85      & 91         & 65 & 67\\
& OracleMap-Waypoints & 80 & 88 & 38 & 39\\
& NoMap & 39      & 59         & 25 & 31\\
& HTP-NearestFrontier & 41 & 54 & 17 & 20\\
% & HTP-GCN\\
& HTP-CNN                       & {\bf 55}    & {\bf 68}    & {\bf 26}    & {\bf 30}\\
& HTP-GCN & 46 & 58 & 19 & 22\\
\midrule
\parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{Hard}}}
& OracleMap (Occ) & 3.6   & 17    & 2.3   & 10\\
& OracleMap (Occ+Obj) & 46      & 69         & 29 & 38\\
& OracleMap-Waypoints & 48 & 72 & 18 & 24\\
& NoMap & 5.2      & 24         & 2.6 & 10\\
& HTP-NearestFrontier & 22 & 40 & 8.1 & 14\\
& HTP-CNN                              & {\bf 33}      & {\bf 53}         & {\bf 13} & {\bf 20}\\
& HTP-GCN & 27 & 47 & 9.4 & 16\\
\midrule
\parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{Harder}}}
& OracleMap (Occ) & 2     & 12    & 1.3   & 7.7\\
& OracleMap (Occ+Obj) & 26      & 48         & 16 & 26\\
& OracleMap-Waypoints & 31 & 59 & 12 & 19\\
& NoMap & 2.8      & 16         & 1.3 & 8.0\\
& HTP-NearestFrontier & 15 & 32 & 5.5 & 12\\
& HTP-CNN & 21      & {\bf 42}         & {\bf 8.6} & {\bf 16}\\ 
& HTP-GCN & {\bf 22} & 39 & 8.0 & 14\\ 
\bottomrule
\end{tabular}
% }
\end{table}


==> tables/multion_results.tex <==
\begin{table}[]
\caption{MultiOn benchmark (standard set) results for 3-object navigation}
\label{tab:multion}
\centering
% \resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
Model & \%Success$\uparrow$ & \%Progress$\uparrow$  & SPL$\uparrow$ & PPL$\uparrow$\\\midrule
OracleMap (Occ) & 16 & 36 & 12 & 27\\
OracleMap (Occ+Obj) & 48 & 62 & 38 & 49\\
NoMap               & 10 & 24 & 4 & 14 \\
FRMQN\cite{frmqn} & 13 & 29 & 24 & 24\\
SMT\cite{fang2019scene} & 9 & 22 & 7 & 18\\
ProjNeuralMap\cite{wani2020multion} & 27 & 46 & 18 & 31\\
ObjRecogMap\cite{wani2020multion} & 22 & 40 & 17 & 30\\
Lyon\cite{marza2021teaching} & 57 & 70 & \textbf{36} & \textbf{45}\\
HTP-CNN (Ours) & 56 & 69 & 30 & 36\\
HTP-GCN (Ours)& \textbf{57} & \textbf{70} & 27 & 33 \\
\bottomrule

\end{tabular}
% }
\end{table}
